Some improvements on Moment-of-Fluid method in 3D rectangular hexahedrons

The moment-of-fluid method (MOF) is an extension of the volume-of-fluid method with piecewise linear interface construction (VOF-PLIC). In MOF reconstruction, the optimized normal vector is determined from the reference centroid and the volume fraction by iteration. The state-of-art work by \citet{milcent_moment--fluid_2020} proposed an analytic gradient of the objective function, which greatly reduces the computational cost. In this study, we further accelerate the MOF reconstruction algorithm by using Gauss-Newton iteration instead of Broyden-Fletcher-Goldfarb-Shanno (BFGS) iteration. We also propose an improved initial guess for MOF reconstruction, which improves the efficiency and the robustness of the MOF reconstruction algorithm. Our implementation of the code and test cases are available on our Github repository.

==> figures.tex <==
%<*fig:distribution>
\begin{figure}[htb]
    \centering
    \subfigure[Exponential case]
    {\includegraphics[width=0.3\textwidth]{dataset2.pdf}}
    \subfigure[Uniform case]
    {\includegraphics[width=0.3\textwidth]{dataset1.pdf}}
    \subfigure[Extreme case]
    {\includegraphics[width=0.3\textwidth]{dataset3.pdf}}
    \caption{Distributions of volume fraction for three data sets.
    }
    \label{fig:distribution}
\end{figure}
%</fig:distribution>

%<*fig:flood>
\begin{figure}[htb]
    \centering
    \subfigure[Evolution with fixed angle]
    {\includegraphics[width=0.33\textwidth]{evo_angle.pdf}}
    \subfigure[Locus of centroids]
    {\includegraphics[width=0.33\textwidth]{flood.pdf}}
    \subfigure[Evolution with fixed volume fraction]
    {\includegraphics[width=0.33\textwidth]{evo_phi.pdf}}
    \caption{The locus of the centroids for reference with fixed volume fraction $V$ (Dashed line)  
     and the locus of cenroids with fixed azimuthal angle $\Phi$ (Solid lines) in a unit 2D cell.
    The black curve corresponds with the locus of centroids for reference volume $V=0.5$.
    }
    \label{fig:flood}
\end{figure}
%</fig:flood>

%<*fig:initialguess>
\begin{figure}[htb]
    \centering
    \subfigure[Initial guess Error of Eq. \eqref{eq:initialguess_1}]
    {\includegraphics[width=0.33\textwidth]{initial_error.pdf}}
    \subfigure[Initial guess Error of Eq. \eqref{eq:initialguess_2}]
    {\includegraphics[width=0.33\textwidth]{initial_error2.pdf}} 
    \subfigure[Initial guess Error of Eq. \eqref{eq:initialguess_3}]
    {\includegraphics[width=0.33\textwidth]{initial_error_hybrid.pdf}} 
    \caption{The azimuthal angle error $\Delta \Theta $ between the initial guess and exact angle.
    }
    \label{fig:initialguess}
\end{figure}
%</fig:initialguess>

==> tables.tex <==
%<*tab:time>
\begin{table}[]
\centering
\caption{Run-time ratio and iteration steps in reconstruction test}
\label{tab:time}
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{Gauss-Newton}                                                                                                                                                                                & \multicolumn{3}{|c}{BFGS}                                                                                                                                                                  \\ \cline{2-7} 
\multicolumn{1}{c}{}                  & \begin{tabular}[c]{@{}l@{}}Averaged\\ iteration\end{tabular} & \begin{tabular}[c]{@{}l@{}}Averaged\\  line search\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}run-time \\ ratio\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Averaged\\ iteration\end{tabular} & \begin{tabular}[c]{@{}l@{}}Averaged\\  line search\end{tabular} & \begin{tabular}[c]{@{}l@{}}run-time \\ ratio\end{tabular} \\ \hline
Original initial guess                & 3.34                                                         & 0                                                               & 1.38                                                                           & 6.26                                                         & 12.56                                                           & 5.29                                                      \\
Improved initial guess                & 2.48                                                         & 0                                                               & 1                                                                              & 5.4                                                          & 10.05                                                           & 4.25                                                      \\ \hline
\end{tabular}
\end{table}
%</tab:time>

%<*tab:error>
\begin{table}[]
\centering
\caption{tab: $L_1$ error of the reconstruction test}
\label{tab:Error}

% Please add the following required packages to your document preamble:

\begin{tabular}{lllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{Gauss-Newton}                      & \multicolumn{3}{|c}{BFGS}         \\ \cline{2-7} 
\multicolumn{1}{c}{}                  & exponential & uniform  & \multicolumn{1}{l|}{extreme} & exponential & uniform  & extreme  \\ \hline
Original initial guess                & 1.98e-09    & 2.92e-06 & 1.19e-05                     & 2.08e-09    & 2.27e-09 & 2.74e-09 \\
Improved initial guess                & 1.97e-09    & 1.93e-09 & 1.85e-09                     & 2.08e-09    & 2.01e-09 & 1.93e-09 \\ \hline
\end{tabular}

\end{table}
%</tab:error>

%<*tab:zalesak>
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{Run time ration and iteration in advection test (Zalesak's problem)}
\label{tab:Zalesak}
\begin{tabular}{@{}lllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{3}{c}{Gauss-Newton}                      & \multicolumn{3}{|c}{BFGS}         \\ \cline{2-7} 
\multicolumn{1}{c}{}                  & \begin{tabular}[c]{@{}l@{}}Averaged\\ iteration\end{tabular} & \begin{tabular}[c]{@{}l@{}}Averaged\\  line search\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}run-time \\ ratio\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Averaged\\ iteration\end{tabular} & \begin{tabular}[c]{@{}l@{}}Averaged\\  line search\end{tabular} & \begin{tabular}[c]{@{}l@{}}run-time \\ ratio\end{tabular} \\ \hline
                    %   & Gauss-Newton                                                 &                                                                 & \multicolumn{1}{l|}{}                                                          & BFGS                                                         &                                                                 &                                                           \\ \midrule
                    %   & \begin{tabular}[c]{@{}l@{}}Averaged\\ iteration\end{tabular} & \begin{tabular}[c]{@{}l@{}}Averaged\\  line search\end{tabular} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}run-time \\ ratio\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Averaged\\ iteration\end{tabular} & \begin{tabular}[c]{@{}l@{}}Averaged\\  line search\end{tabular} & \begin{tabular}[c]{@{}l@{}}run-time \\ ratio\end{tabular} \\ \midrule
Grid: $50\times50\times50$                   &                                                              &                                                                 &                                                                                &                                                              &                                                                 &                                                           \\
Original initial guess & 3.68                                                         & 0                                                               & 1.06                                                                           & 6.86                                                         & 17.09                                                           & 3.38                                                \\
Improved initial guess & 3.29                                                         & 0                                                               & 1                                                                              & 5.35                                                         & 10.87                                                           & 2.73                                               \\ \midrule
Grid: $100\times100\times100$                   &                                                              &                                                                 &                                                                                &                                                              &                                                                 &                                                           \\
Original initial guess & 3.79                                                         & 0                                                               & 1.15                                                                           & 7.03                                                         & 16.76                                                           & 3.18                                               \\
Improved initial guess & 3.37                                                         & 0                                                               & 1                                                                              & 5.91                                                         & 10.17                                                           & 2.92                                               \\ \bottomrule
\end{tabular}
\end{table}
%</tab:zalesak>
